Bellwethers: A Baseline Method For Transfer Learning

Software analytics builds quality prediction models for software projects. Experience shows that (a) the more projects studied, the more varied are the conclusions; and (b) project managers lose faith in the results of software analytics if those results keep changing. To reduce this conclusion instability, we propose the use of "bellwethers": given N projects from a community the bellwether is the project whose data yields the best predictions on all others. The bellwethers offer a way to mitigate conclusion instability because conclusions about a community are stable as long as this bellwether continues as the best oracle. Bellwethers are also simple to discover (just wrap a for-loop around standard data miners). When compared to other transfer learning methods (TCA+, transfer Naive Bayes, value cognitive boosting), using just the bellwether data to construct a simple transfer learner yields comparable predictions. Further, bellwethers appear in many SE tasks such as defect prediction, effort estimation, and bad smell detection. We hence recommend using bellwethers as a baseline method for transfer learning against which future work should be compared

==> figures/defect_results.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/apache.png}
    \caption[]%
    {{\small }}    
    \label{fig:mean and std of net14}
\end{figure}


==> figures/effort_results.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/cocomodata.png}
    \caption[]%
    {{\small }}    
    \label{fig:mean and std of net14}
\end{figure}


==> figures/smells_results.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/godclass.png}
        \caption[]%
        {{\small }}    
        \label{fig:mean and std of net14}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{figures/featureenvy.png}
        \caption[]%
        {{\small}}    
        \label{fig:mean and std of net24}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures/dataclass.png}
        \caption[]%
        {{\small}}    
        \label{fig:mean and std of net34}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures/longmethod.png}
        \caption[]%
        {{\small}}    
        \label{fig:smells}
    \end{subfigure}
    \caption[]
    {\small A comparative study of transfer learners in predicting code smells from the Qualitas Corpus.} 
    \label{fig:mean and std of nets}
\end{figure*}


==> name.tex <==
Software analytic builds quality prediction models
for software projects. Experience shows that (a) the more projects studied, the more
varied are the conclusions; and (b)
project managers lose faith in the results of software analytics if those results keep changing
To reduce  this  conclusion instability,
we propose  ``bellwethers'': given N projects from a community  the bellwether
is the   project whose data     
yields   best predictions on all  others. The bellwethers offer a way to tame conclusion stability because conclusions about a community are stable as long as this bellwether continues as the best oracle. Bellwethers are also simple to discover (just wrap a for-loop around standard data miners). When compared to other  transfer learning methods  (TCA+,
 transfer Naive Bayes, value cognitive boosting), using just the bellwether data to construct a simple transfer learner yields better predictions in several cases.
Further, bellwethers appear in many SE tasks such as defect prediction, effort estimation, bad smell detection and predicting issue lifetime. We hence recommend using bellwethers as a {\em baseline method} for transfer learning against which  future work should be compared.

==> tex/aeeem.tex <==
\begin{figure*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{{EQ}} &  & & & \\\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           LC &    0.34  &  0.02 & \quart{41}{3}{43}{126} \\
  1 &           ML &    0.35  &  0.01 & \quart{43}{1}{44}{126} \\
\hline  2 &          PDE &    0.4  &  0.02 & \quart{49}{3}{50}{126} \\
\hline  3 &          JDT &    0.62  &  0.01 & \quart{78}{1}{78}{126} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{JDT} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           LC &    0.28  &  0.0 & \quart{60}{0}{60}{216} \\
  1 &          PDE &    0.28  &  0.01 & \quart{58}{2}{60}{216} \\
  1 &           ML &    0.28  &  0.03 & \quart{60}{7}{60}{216} \\
\hline  2 &           EQ &    0.36  &  0.02 & \quart{75}{4}{77}{216} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{ML} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           LC &    0.37  &  0.01 & \quart{56}{2}{58}{156} \\
\hline  2 &          PDE &    0.39  &  0.02 & \quart{59}{3}{61}{156} \\
\hline  3 &           EQ &    0.42  &  0.01 & \quart{65}{2}{65}{156} \\
\hline  4 &          JDT &    0.51  &  0.01 & \quart{78}{1}{79}{156} \\
\hline \end{tabular}}\\[0.45cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{PDE} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           EQ &    0.32  &  0.0 & \quart{45}{0}{45}{142} \\
\hline  2 &           ML &    0.34  &  0.02 & \quart{47}{2}{48}{142} \\
\hline  3 &           LC &    0.36  &  0.02 & \quart{49}{3}{51}{142} \\
\hline  4 &          JDT &    0.54  &  0.05 & \quart{72}{7}{77}{142} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{LC} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           EQ &    0.27  &  0.01 & \quart{39}{2}{41}{153} \\
\hline  2 &          PDE &    0.34  &  0.02 & \quart{50}{3}{52}{153} \\
\hline  3 &           ML &    0.4  &  0.05 & \quart{56}{8}{61}{153} \\
\hline  4 &          JDT &    0.51  &  0.02 & \quart{76}{3}{78}{153} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{CM} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.37  &  0.0 & \quart{42}{0}{42}{115} \\
  1 &           jm &    0.41  &  0.0 & \quart{47}{0}{47}{115} \\
\hline  2 &           mw &    0.49  &  0.0 & \quart{56}{0}{56}{115} \\
\hline  3 &           kc &    0.69  &  0.0 & \quart{79}{0}{79}{115} \\
\hline \end{tabular}}\\[0.45cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{JM} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.38  &  0.0 & \quart{39}{0}{39}{103} \\
\hline  2 &           kc &    0.65  &  0.0 & \quart{67}{0}{67}{103} \\
\hline  3 &           mw &    0.69  &  0.0 & \quart{71}{0}{71}{103} \\
\hline  4 &           cm &    0.77  &  0.0 & \quart{79}{0}{79}{103} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{KC} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.4  &  0.0 & \quart{40}{0}{40}{101} \\
\hline  2 &           jm &    0.44  &  0.0 & \quart{44}{0}{44}{101} \\
\hline  3 &           mw &    0.59  &  0.0 & \quart{59}{0}{59}{101} \\
\hline  4 &           cm &    0.79  &  0.0 & \quart{79}{0}{79}{101} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{MW} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.32  &  0.0 & \quart{41}{0}{41}{129} \\
\hline  2 &           kc &    0.41  &  0.0 & \quart{52}{0}{52}{129} \\
\hline  3 &           jm &    0.57  &  0.0 & \quart{73}{0}{73}{129} \\
\hline  4 &           cm &    0.62  &  0.0 & \quart{79}{0}{79}{129} \\
\hline \end{tabular}}\\[0.45cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Apache} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &         Safe &    0.47  &  0.0 & \quart{72}{0}{72}{153} \\
  1 &        Zxing &    0.51  &  0.09 & \quart{66}{13}{78}{153} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{ZXing} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &         Safe &    0.51  &  0.0 & \quart{51}{0}{51}{101} \\
\hline  2 &       Apache &    0.79  &  0.0 & \quart{79}{0}{79}{101} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Safe} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &        Zxing &    0.3  &  0.03 & \quart{39}{5}{42}{142} \\
\hline  2 &       Apache &    0.56  &  0.0 & \quart{79}{0}{79}{142} \\
\hline \end{tabular}}

\caption{Prediction performance in Apache Dataset}
\label{fig:aeeem}
\end{figure*}

==> tex/codeattr.tex <==
\begin{figure}[t!]
% \arrayrulecolor{lightgray}
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{c|p{0.8in}|p{1.8in}}
wmc & weighted methods per class & \\\hline
dit & depth of inheritance tree & \\\hline
noc &  number of children & \\\hline
cbo & coupling between objects & increased when the methods of one
class access services of another. \\\hline
rfc & response for a class &number of  methods invoked in response to
a message to the object. \\\hline
lcom & lack of cohesion in methods &number of pairs of methods that do
not share a reference to an instance variable. \\\hline
ca & afferent couplings & how many other classes use the specific
class.  \\\hline
ce & efferent couplings & how many other classes is used by the
specific class.  \\\hline
npm & number of public methods &  \\\hline
locm3 & another lack of cohesion measure & if $m,a$ are  the number of
$methods,attributes$
in a class number and $\mu(a)$  is the number of methods accessing an
attribute, 
then
$lcom3=((\frac{1}{a} \sum_j^a \mu(a_j)) - m)/ (1-m)$.
 \\\hline
loc & lines of code & \\\hline
dam & data access & ratio of  private (protected)
attributes to   total   attributes \\\hline
moa &  aggregation &  count of the number of data declarations (class
fields) whose types are user defined classes \\\hline
mfa & functional abstraction & number of methods inherited by a class
plus number of methods accessible by member methods of the
class \\\hline
cam & cohesion amongst classes & summation of number of different
types of method parameters in every method divided by a multiplication
of number of different method parameter types in whole class and
number of methods.  \\\hline
ic & inheritance coupling &  number of parent classes to which a given
class is coupled (includes counts of methods and variables inherited)
\\\hline
cbm &coupling between methods &  total number of new/redefined methods
to which all the inherited methods are coupled \\\hline
amc & average method complexity & e.g. number of JAVA byte codes \\\hline
max\_cc & maximum McCabe & maximum McCabe's cyclomatic complexity seen
in class \\\hline
avg\_cc & average McCabe & average McCabe's cyclomatic complexity seen
in class \\\hline
\rowcolor{lightgray}
defect & defect & Boolean: where defects found in post-release bug-tracking systems.
\end{tabular}
} 
\caption{Sample static code attributes.}\label{fig:ck}
\end{figure}


==> tex/defects_dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Community}} & \multicolumn{1}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{2}{c|}{\# of instances} & \multicolumn{1}{c|}{\multirow{2}{*}{\# metrics}} & \multicolumn{1}{c}{\multirow{2}{*}{Nature}} \bigstrut\\ \cline{3-4}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Total} & \multicolumn{1}{c|}{Bugs (\%)} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} \bigstrut\\ \hline
\multirow{5}{*}{AEEEM} & EQ & 325 & 129 (39.81) & \multirow{5}{*}{61} & \multirow{5}{*}{Class} \\
 & JDT & 997 & 206 (20.66) &  &  \\
 & LC & 399 & 64 (9.26) &  &  \\
 & ML & 1826 & 245 (13.16) &  &  \\
 & PDE & 1492 & 209 (13.96) &  &  \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Relink}} & Apache & 194 & 98 (50.52) & \multirow{3}{*}{26} & \multirow{3}{*}{File} \\
\multicolumn{1}{c|}{} & Safe & 56 & 22 (39.29) &  &  \\
\multicolumn{1}{c|}{} & ZXing & 399 & 118 (29.57) &  &  \\ \hline
\multirow{10}{*}{Apache} & Ant & 1692 & 350 (20.69) & \multirow{10}{*}{20} & \multirow{10}{*}{Class} \\
 & Ivy & 704 & 119 (16.90) &  &  \\
 & Camel & 2784 & 562 (20.19) &  &  \\
 & Poi & 1378 & 707 (51.31) &  &  \\
 & Jedit & 1749 & 303 (17.32) &  &  \\
 & Log4j & 449 & 260 (57.91) &  &  \\
 & Lucene & 782 & 438 (56.01) &  &  \\
 & Velocity & 639 & 367 (57.43) &  &  \\
 & Xalan & 3320 & 1806 (54.40) &  &  \\
 & Xerces & 1643 & 654 (39.81) &  &  \\ \hline
\multirow{5}{*}{NASA} & cm & 998 & 126 (12.63) & \multirow{5}{*}{23} & \multirow{5}{*}{Function} \\
 & jm & 25157 & 5103 (20.28) &  &  \\
 & kc & 588 & 108 (18.37) &  &  \\
 & mc & 13630 & 292 (2.14) &  &  \\
 & mw & 770 & 81 (10.52) &  &  \\ \hline
\end{tabular}%
}
\caption{59 Defect Datasets from 4 communities.
The \# metrics columns shows the number of metrics that are shared
by all members of that community. }
\label{fig:defects_dataset}
\end{figure}

==> tex/effort_dataset.tex <==
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\hline
Community               & Dataset  & Samples & Range (min-max) & \# metrics          & Nature                            \\ \hline
\multirow{5}{*}{Effort} & Mystery2 & 95      & 3.5 - 2673    & \multirow{5}{*}{24} & \multirow{5}{*}{FP} \\ \cline{2-4}
                        & nasa93   & 93      & 8.4 - 8211    &                     &                                   \\ \cline{2-4}
                        & coc81    & 63      & 5.9 - 11400   &                     &                                   \\ \cline{2-4}
                        & Mystery1 & 17      & 320 - 3291.8  &                     &                                   \\ \cline{2-4}
                        & cocomo   & 12      & 1 - 22      &                     &                                   \\ \hline
\end{tabular}}
\caption{5 Effort Estimation data sets measured in terms of functional points analysis.
The \# metrics columns shows the number of metrics that are shared
by all members of that community.}
\label{fig:effort_dataset}
\end{figure}

==> tex/expt_setup.tex <==
\begin{figure}[tb!]
\centering
\begin{tabular}{|p{0.95\linewidth}|} \hline
\\[-0.2cm]
\textbf{\ref{fig:expt_setup}.A: Discovering the bellwether. }
\be
    \item For each community in every sub-domain, we pick a project $P_i$. We use this as the training set to construct a quality prediction model according to the learning method described in \tion{met}.
    \item Next, we pick another project $P_j \notin P_i$ and retain this as a holdout dataset.
    \item Then, for every other project $P_k$ where $k \in {1,\dots,n};~k\notin \{i,j\}$, that belong to the same community as $\{P_i, P_j\}$, we evaluate the performance of $P_i$ for $P_k$ according to the evaluation strategy discussed in \tion{eval}. 
    \item We repeat steps 1,2, and 3 for all pairs of projects in a community. 
    \ee
This whole process is repeated 30 times, with different random number seeds. Then, we use the statistical test described in \tion{stats} to rank each project $P_i$. For every holdout dataset in step 2 above, if there exists one project that returns consistently high performance scores, we label that as the bellwether.

\\[-.2cm]\hline
\\[-.2cm]
\textbf{\ref{fig:expt_setup}.B: Discovering the best transfer learner.}
\be
    \item For each community in every sub-domain, we pick a project $P_i$ as in \fig{expt_setup}.A. We then use this as the training data to construct the transfer learners (TCA+, TNB, VCB, and Bellwether Method).
    \item For every other project $P_j$ where $j \in {1,\dots,n};~j\notin i$, that belong to the same community as $P_i$, we evaluate the performance of each of the transfer learners and use the evaluation strategy discussed in \tion{eval} to evaluate their performance. 
\ee
Similar to above, the above steps are repeated 30 times, with different random number seeds. Then, we use the statistical test  from \tion{stats} to rank each transfer learner.
\\[0.1cm]
\hline
\end{tabular}
\caption{\respto{2-C-2} Experimental setup. Note: figure~\ref{fig:loo} uses the the procedure described in~\fig{expt_setup}. Figures~\ref{fig:smells_result}, \ref{fig:issues_result}, \ref{fig:defects_results}, and~\ref{fig:effort_result} uses setup described in \ref{fig:expt_setup}.B.}
\label{fig:expt_setup}
\end{figure}

==> tex/graph_sample.tex <==
\begin{figure}[tb!]
\centering
\begin{tabular}{|p{0.9\linewidth}|} \hline
\hspace{0.15\linewidth}\includegraphics[width=.7\linewidth]{figures/success1.png}
\\
\fig{graph_sample}.A: In this first example figure, the thick line shows the bellwether results and the dotted lines show results  from other transfer learning methods.
The key feature of this figure is that the for the data sets A,B,C,D...L, the thick Bellwether line falls outside all the rest. That is, results like this can be summarized as ``bellwether performs {\em \underline{better}}  than the other transfer learning methods''.
\\\hline
\hspace{0.15\linewidth}\includegraphics[width=.7\linewidth]{figures/fails.png}
\\
\fig{graph_sample}.B: In this second example figure,  for the data sets A,B,C,D...L, the thick Bellwether line often falls inside all the rest. That is, results like this can be summarized as ``bellwether often performs {\em \underline{worse}} than the other transfer learning methods''.
\\\hline
\end{tabular}
 
\caption{Reference charts (with contrived values) shows bellwether succeeding and failing.}
\label{fig:graph_sample}
\end{figure}

==> tex/issues_dataset.tex <==
\begin{figure}[t]
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l}
  \hline
  \multirow{2}{*}{Dataset}      & \multirow{2}{*}{Days} & \multicolumn{2}{c|}{\# of instances} & \multirow{2}{*}{\# metrics} \\ \cline{3-4}
  &                       & Total                  & Closed (\%) &                             \\ \hline
\multirow{5}{*}{camel}        & 1 day   & \multirow{5}{*}{5056} & 698 (14.0) & \multirow{5}{*}{18} \\
& 7 days  &                       & 437 (9.0)  &                     \\
& 14 days &                       & 148 (3.0)  &                     \\
& 30 days &                       & 167 (3.0)  &                     \\
& 90 days &                       & 300 (6.0)  &                     \\ \hline
\multirow{5}{*}{cloudstack}   & 1 day   & \multirow{5}{*}{1551} & 658 (42.0) & \multirow{5}{*}{18} \\
& 7 days  &                       & 457 (29.0) &                     \\
& 14 days &                       & 101 (7.0)  &                     \\
& 30 days &                       & 107 (7.0)  &                     \\
& 90 days &                       & 133 (9.0)  &                     \\ \hline
\multirow{5}{*}{cocoon}       & 1 day   & \multirow{5}{*}{2045} & 125 (6.0)  & \multirow{5}{*}{18} \\
& 7 days  &                       & 92 (4.0)   &                     \\
& 14 days &                       & 32 (2.0)   &                     \\
& 30 days &                       & 45 (2.0)   &                     \\
& 90 days &                       & 85 (4.0)   &                     \\ \hline
\multirow{5}{*}{deeplearning} & 1 day   & \multirow{5}{*}{1434} & 931 (65.0) & \multirow{5}{*}{18} \\
& 7 days  &                       & 214 (15.0) &                     \\
& 14 days &                       & 76 (5.0)   &                     \\
& 30 days &                       & 72 (5.0)   &                     \\
& 90 days &                       & 69 (5.0)   &                     \\ \hline
\multirow{5}{*}{hadoop} & 1 day   & \multirow{5}{*}{12191} & 40 (0.0)    & \multirow{5}{*}{18} \\
& 7 days  &                        & 65 (1.0)    &                     \\
& 14 days &                        & 107 (1.0)   &                     \\
& 30 days &                        & 396 (3.0)   &                     \\
& 90 days &                        & 1744 (14.0) &                     \\ \hline
\multirow{5}{*}{hive}   & 1 day   & \multirow{5}{*}{5648}  & 18 (0.0)    & \multirow{5}{*}{18} \\
& 7 days  &                        & 22 (0.0)    &                     \\
& 14 days &                        & 58 (1.0)    &                     \\
& 30 days &                        & 178 (3.0)   &                     \\
& 90 days &                        & 1051 (19.0) &                     \\ \hline
\multirow{5}{*}{ofbiz}  & 1 day   & \multirow{5}{*}{6177}  & 1515 (25.0) & \multirow{5}{*}{18} \\
& 7 days  &                        & 1169 (19.0) &                     \\
& 14 days &                        & 467 (8.0)   &                     \\
& 30 days &                        & 477 (8.0)   &                     \\
& 90 days &                        & 577 (9.0)   &                     \\ \hline
\multirow{5}{*}{qpid}   & 1 day   & \multirow{5}{*}{5475}  & 203 (4.0)   & \multirow{5}{*}{18} \\
& 7 days  &                        & 188 (3.0)   &                     \\
& 14 days &                        & 84 (2.0)    &                     \\
& 30 days &                        & 178 (3.0)   &                     \\
& 90 days &                        & 559 (10.0)  &                     \\ \hline
\end{tabular}}
\caption{}
\label{fig:issues_dataset}
\end{figure}

==> tex/nasa.tex <==
\begin{figure}[htbp!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
 & CM & JM & KC & MC & MW \\ \hline
CM &  &  &  & $\times$ &  \\ \hline
JM &  &  &  & $\times$ &  \\ \hline
KC &  &  &  & $\times$ &  \\ \hline
MW &  &  &  & $\times$ &  \\ \hline
MC &  & $\times$ &  &  & 
\end{tabular}~~~\begin{tabular}{l|l|l|l|l|l}
 & EQ & JDT & LC & ML & PDE \\ \hline
EQ &  &  & $\times$ &  &  \\ \hline
JDT &  &  & $\times$ &  &  \\ \hline
ML &  &  & $\times$ &  &  \\ \hline
PDE & $\times$ &  &  &  &  \\ \hline
LC & $\times$ &  &  &  & 
\end{tabular}~~~\begin{tabular}{l|l|l|l}
 & Apache & ZXing & Safe \\ \hline
Apache &  &  & $\times$ \\ \hline
ZXing &  &  & $\times$ \\ \hline
Safe &  & $\times$ & 
\end{tabular}}
\caption{Bellwether Effect}
\label{fig:nasa}
\end{figure}

==> tex/oo2.tex <==
\begin{figure*}[!t]
\begin{center}
\resizebox{.67\linewidth}{!}{
{\footnotesize\begin{tabular}{r|r|r|r|r|r|r|r|l|l}\hline
ref & cbo & 
rfc & 
lcom & 
dit & 
noc & 
wmc & 
\begin{sideways}\#projects\end{sideways} & 
size & type\\\hline
\cite{ref01} & + & + & + & - & - & + & 6 & 95-201  & 6 versions of rhino (java)\\
\cite{ref02} & + & + & + & - & - & + & 12 & 86 classess (3-12kloc) & student\\
\cite{ref03} & + & + & - &  &  &  & 1 & 1700  (110kloc) & commercial telecom\\
\cite{ref04} & + & + & - & + & + & + & 8 & 113  & student\\
\cite{ref05} & + & + & - & + & + & + & 8 & 114  & student\\
\cite{ref06} & + & + & + & + & - &  & 1 & 83  & commercial: lalo (c++)\\
\cite{ref07} &  &  &  & + & + &  & 1 & 32  & commercial: telecom c++\\
\cite{ref08} &  &  &  & + & - &  & 1 & 42-69  & commercial java word proc.\\
\cite{ref09} & + & - & - & - & - & - & 1 & 85  & telecom c++\\
\cite{ref10} & - & + &  & - & - & + & 3 & 92  & 3 c++ subsystems,commercial\\
\cite{ref11} & + & + & + & - & + & + & 1 & 123  (34kloc) & java commercial\\
\cite{ref12} & + &  &  & + &  & + & 1 & 706  & commercial c++ and java\\
\cite{ref13} & + & + & + & - & + & + & 1 & 145  & kc1-nasa\\
\cite{ref14} & + & + & + & + & - & + & 1 & 3677  & open source:mozilla\\
\cite{ref15} & + & + & + &  &  & + & 1 & ? & java (sap) commercial\\
\cite{ref16} & + & + & + & + & + & + & 3 & ? & eclipse 2.0, 2.1, 3.0\\
\cite{ref17} & - & + & + & - & - & + & 8 & 113  & student\\
\cite{ref18} &  & + & + & + & + &  & 2 & 64  & sales and cd-selection system\\
\cite{ref19} &  & - &  & - & - & - & 1 & 3344 modules (2mloc) & commercial telecom c++\\
\cite{ref20} & + & + & + & - & - & + & 5 & 395  & commercial telecom c++\\
\cite{ref21} & + & + &  & - & - & + & 1 & 1412  & open source:jdt\\
\cite{ref22} & + & + &  & - & - & + & 2 & 9713  & eclipse 2.0, 2.1\\
\cite{ref23} & + & + & - & - & - & + & 1 & 145  & kc1-nasa\\
\cite{ref24} &  &  &  & + & - &  & 1 & 145  & commercial java xml editor\\
\cite{ref25} & - & - & - & - & - & - & 1 & 174  & commercial telecom c++\\
\cite{ref26} & - &  &  &  &  & - & 0 & 50  & student\\
\cite{ref27} & + & + & - & - & - & + & 1 & 145  & kc1-nasa\\
\cite{ref28} &  & + &  & + & + &  & 2 & 294  & commercial c++\\\hline
total +  & 18 & 20 & 11 & 11 & 8 & 17\\\cline{1-7} 
total -  & 4 & 3 & 7 & 14 & 16 & 4&\multicolumn{1}{r}{KEY:}&\multicolumn{2}{l}{\colorbox{green}{Strong consensus (over 2/3rds)}}\\\cline{1-7}
\multicolumn{2}{l}{Total percents:}&\multicolumn{5}{r}{ ``*'' denotes majority conclusion  in each column}&\multicolumn{1}{r}{~}&\multicolumn{2}{l}{\colorbox{yellow}{Some consensus (less than 2/3rds)}}\\\cline{1-7}
 + & \cellcolor{yellow}* 64\%	&\cellcolor{green}* 71\%&	\cellcolor{pink}* 39\%&	39\%&	29\%&	\cellcolor{yellow}* 61\%&\multicolumn{1}{c}{~}&\multicolumn{2}{l}{\colorbox{lightgray}{Weak consensus (about half)}}\\\cline{1-7}
 - & 14\%&	11\%&	25\%&\cellcolor{lightgray}* 50\%&	\cellcolor{lightgray}* 57\%&	14\%&\multicolumn{1}{c}{~}&\multicolumn{2}{l}{\colorbox{pink}{No consensus }}\\\cline{1-7}
\end{tabular}}}
\renewcommand{\arraystretch}{1}
\end{center}
\caption{ Contradictory conclusions from OO-metrics studies for defect
  prediction. Studies report significant (``+'') or irrelevant (``-'')
  metrics verified by univariate prediction models. Blank
  entries indicate that the corresponding metric is not evaluated in
  that particular study. Colors comment on the most frequent conclusion
  of each column. CBO= coupling between objects; RFC= response
  for class (\#methods executed by arriving messages); LCOM= lack of
  cohesion (pairs of methods referencing one instance variable,
  different definitions of LCOM are aggregated); NOC= number of
  children (immediate subclasses); WMC= \#methods per class. }\label{fig:turhan}
\end{figure*}


==> tex/pseudo-code-1.tex <==
\begin{figure}[t]

\begin{python}
def kNN(training, testing, F=33):
  "Identify contrast sets for testing
      data using Nearest Neighbor "
  def exemplar(rows):
    return centroid(rows)
  
  def nearest(me, clusters):
    return sorted(clusters,
                  key=lambda F: dist(exemplar(F), me))
  
  def envy(me, clusters):
    one=exemplar(nearest(me, clusters))
    better=[c for c in clusters if score(c)<score(one)]
    two=exemplar(nearest(one, better))
    return one, two
  
  def FSel(list, Frac):
    "Return top Frac % of the list"
    
  def contrastSet(t):
    clusters = WHERE(training)
    one, two = envy(t,clusters)
    return FSel(one-two, Frac=F)
  
  # ---- Begin Main Code ---------------
  return [contrastSet(t) for t in testing]
\end{python}
\caption{Nearest Neighbor (Python-style psuedo-code).
For brevity's sake, this code skips certain low-level details.
For a full working implementation, see \url{http://git.io/v36sb}.}
\label{fig:knncode}
\end{figure}

==> tex/refactor.tex <==
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 
\begin{figure}[!t] 
\scriptsize
\centering
\begin{tabular}{r|c|c|c|c} 


\begin{turn}{75}Fowler'99~\cite{fowler99} and~\cite{Kerievsky2005}\end{turn} &\begin{turn}{75} Lanza'06~\cite{Lanza2006}\end{turn} & \begin{turn}{75}SonarQube~\cite{sq15} \end{turn} &  \begin{turn}{75}Yamashita'13\cite{Yamashita2013} \end{turn}& \begin{turn}{75} Developer Survey 2015\end{turn}\\\hline
  Alt. Classes with Diff. Interfaces & & & & \\
  Combinatorial Explosion~\cite{Kerievsky2005} & & &  & \\
  Comments & & & 11 & VL\\
  Conditional Complexity~\cite{Kerievsky2005} & & & 14  & ?\\
  Data Class & \checkmark & &  &\\
  Data Clumps &  &  &  &\\
  Divergent Change & & &  & \\
  Duplicated Code & \checkmark & \checkmark & 1  & VH\\
  Feature Envy & \checkmark & & 8  &\\
  
  Inappropriate Intimacy & & \checkmark &  & L\\
  Indecent Exposure~\cite{Kerievsky2005} & & &  & ?\\
  Incomplete Library Class & & &  &\\
  Large Class & \checkmark & \checkmark & 4  & VH\\
  Lazy Class/Freeloader & & \checkmark & 7  &\\
  Long Method & \checkmark& \checkmark & 2  & VH\\
  Long Parameter List &  & \checkmark & 9  & L \\
  
  Message Chains & & &  & H\\
  Middle Man & &  &  &\\
  Oddball Solution~\cite{Kerievsky2005} & & &  & \\
  Parallel Inheritance Hierarchies & & &  &\\
  Primitive Obsession &  & &  &\\
  
  Refused Bequest & \checkmark & \checkmark &  & \\ 
  Shotgun Surgery & \checkmark& &  & \\
  Solution Sprawl~\cite{Kerievsky2005} & & &  &\\
  Speculative Generality & & &  & L\\
  Switch Statements &  & &  & L\\
  Temporary Field & & \checkmark &  & ?\\
  \end{tabular}
%   \multicolumn{5}{l}{} \\
%   \multicolumn{5}{l}{\textsuperscript{\textdagger} + Exact rule, - Possibly related rule} \\
%     \multicolumn{5}{l}{\textsuperscript{\textdaggerdbl} + is included in list} \\
%     \multicolumn{5}{l}{\textsuperscript{\textexclamdown} VH: Very High, H: High, L: Low, VL: Very Low, ?: Still investigating} \\
%   \multicolumn{5}{l}{\textsuperscript{*} Computation is based on more than simple metrics.} \\

\caption{Bad   smells from different sources.  Check marks (\protect\checkmark) denote   a bad smell was mentioned.
Numbers or symbolic labels (e.g. "VH") denote  a priorization comment (and
``?'' indicates lack of consensus). Empty cells
denote some bad smell listed in column one that was not found relevant
in other studies.
Note: there are many blank cells.}
\label{fig:smells}
\end{figure}

==> tex/results2.tex <==
\begin{figure}[t!]
\arrayrulecolor{darkgray}
\centering
\begin{minipage}[b!]{\linewidth}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\cline{2-6}

&     Source     & Bellwether & \textbf{TCA+}   & TNB   & VCB    \\
   &          & {Method} &   &   \\\hline
\multicolumn{1}{l|}{\multirow{10}{*}{Apache}} & \textbf{Lucene}   & 
63         & 
\cellcolor[HTML]{EFEFEF}\textbf{69}    
& 57    & 64     \\
\multicolumn{1}{l|}{}                           & Xalan    & 57         & 
\cellcolor[HTML]{EFEFEF}64    
& 59    & 62     \\
\multicolumn{1}{l|}{}                           & Camel    & 60         & 
\cellcolor[HTML]{EFEFEF}63    
& 59    & 44     \\
\multicolumn{1}{l|}{}                           & Velocity & 58         & 
\cellcolor[HTML]{EFEFEF}63    
& 51    & 63     \\
\multicolumn{1}{l|}{}                           & Ivy      & 60         & 
\cellcolor[HTML]{EFEFEF}62    
& 61    & 48     \\
\multicolumn{1}{l|}{}                           & Log4j    & 60         & 
\cellcolor[HTML]{EFEFEF}62    
& 58    & 62     \\
\multicolumn{1}{l|}{}                           & Xerces   & 
\cellcolor[HTML]{EFEFEF}57         & 54    
& 58    & 65     \\
\multicolumn{1}{l|}{}                           & Ant      & 
\cellcolor[HTML]{EFEFEF}61         & 52    
& 45    & 55     \\
\multicolumn{1}{l|}{}                           & Jedit    & 
\cellcolor[HTML]{EFEFEF}58         & 43    
& 57    & 49     \\ \cline{2-6} 
\multicolumn{1}{l|}{}                           & W/T/L    & 2/0/7      & 
\cellcolor[HTML]{EFEFEF}\textbf{6/0/3} 
& 0/0/9 & 1/2/06 \\ \hline\hline
\multicolumn{1}{l|}{\multirow{4}{*}{ReLink}}    & \textbf{Zxing}    & 
\cellcolor[HTML]{EFEFEF}\textbf{68}         & \cellcolor[HTML]{EFEFEF}\textbf{67}    
& 53    & 64     \\
\multicolumn{1}{l|}{}                           & Safe     & 
\cellcolor[HTML]{EFEFEF}38         & 34    
& 36    & 31     \\
\multicolumn{1}{l|}{}                           & Apache   & 31         & 31    
& \cellcolor[HTML]{EFEFEF}32    & 31     \\ \cline{2-6} 
\multicolumn{1}{l|}{}                           & W/T/L    & 
\cellcolor[HTML]{EFEFEF}\textbf{0/1/1}      & 0/1/1 
& 1/0/2 & 0/1/2  \\ \hline\hline
\multicolumn{1}{l|}{}                        & \textbf{LC}    & 
\cellcolor[HTML]{EFEFEF}\textbf{75} & \cellcolor[HTML]{EFEFEF}\textbf{75}    & 
73                         & 61                    \\
\multicolumn{1}{l|}{}                        & ML    & 
\cellcolor[HTML]{EFEFEF}73 & \cellcolor[HTML]{EFEFEF}73    & 
67                         & 51                    \\
\multicolumn{1}{l|}{}                        & PDE   & 
70                         & \cellcolor[HTML]{EFEFEF}71    & 
60                         & 57                    \\
\multicolumn{1}{l|}{}                        & JDT   & 
63                         & 64                            & 
\cellcolor[HTML]{EFEFEF}68 & 53                    \\
\multicolumn{1}{l|}{}                        & EQ    & 
59                         & \cellcolor[HTML]{EFEFEF}61    & 
59                         & 57                    \bigstrut\\ \cline{2-6} 
\multicolumn{1}{l|}{\multirow{-6}{*}{AEEEM}} & W/T/L & 
0/2/3                      & \cellcolor[HTML]{EFEFEF}\textbf{2/2/1} & 
1/0/4                      & 0/0/5                 \\ \hline
 \end{tabular}}
\end{minipage}~~
\begin{minipage}[c]{0.5\linewidth}
\resizebox{0.7\linewidth}{!}{%
\hfill
\begin{tabular}{l|l|l|l|l}
\cline{2-5}

& Source & Bellwether                   & TCA                          & TNB   \\ \hline
& cocomo & \cellcolor[HTML]{C0C0C0}0.98 & 0.90                         & 0.90  \\
& nasa93 & \cellcolor[HTML]{C0C0C0}0.93 & 0.85                         & 0.35  \\
& nasa10 & \cellcolor[HTML]{C0C0C0}0.90 & 0.53                         & 0.65  \\
& coc81  & 0.83                         & \cellcolor[HTML]{C0C0C0}0.85 & 0.60  \\
& coc10  & 0.55                         & \cellcolor[HTML]{C0C0C0}0.75 & 0.73  \\ \cline{2-5} 
\multirow{-6}{*}{FPA} & W/T/L  & 3/0/2                        & 2/0/3                        & 0/0/5 \\ \hline


\end{tabular}}
\end{minipage}
\caption{Defect Datasets: This figure compares the prediction performance of the bellwether 
dataset (Lucene,Zxing,LC) against other datasets (other rows). \textit{Bellwether Method} against Transfer Learners (columns) for detecting defects. The numerical value seen here are the median G-scores from Equation 2 over 30 repeats where one dataset is used as a source and others are used as targets in a round-robin fashion.  Higher values are better and cells highlighted in gray produce the best Scott-Knott ranks. The last row in each community indicate Win/Tie/Loss(W/T/L). \textit{TCA+} is the overall best transfer learner.}
\label{fig:defects_results}
\end{figure}

==> tex/rq1.tex <==
\begin{figure*}[t!]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll}
 & \multicolumn{2}{l|}{Ant} & \multicolumn{2}{l|}{Camel} & \multicolumn{2}{l|}{Ivy} & \multicolumn{2}{l|}{Poi} & \multicolumn{2}{l|}{Velocity} & \multicolumn{2}{l|}{Xalan} & \multicolumn{2}{l|}{Xerces} & \multicolumn{2}{l|}{Jedit} & \multicolumn{2}{l|}{Log4j} & \multicolumn{2}{l}{Lucene} \\ \cline{2-21} 
 & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr \\ \hline
Ant &  &  & 0.33 & 0.01 & 0.32 & 0.01 & 0.28 & 0.01 & 0.28 & 0.02 & 0.3 & 0.01 & 0.3 & 0.01 & 0.34 & 0.01 & 0.28 & 0.02 & \cellcolor[HTML]{E8E8E8}0.28 & \cellcolor[HTML]{E8E8E8}0 \\
Camel & 0.61 & 0.01 &  &  & 0.62 & 0.02 & 0.57 & 0.01 & 0.47 & 0.01 & 0.53 & 0.01 & 0.42 & 0.01 & 0.71 & 0.03 & 0.42 & 0.02 & \cellcolor[HTML]{E8E8E8}0.4 & \cellcolor[HTML]{E8E8E8}0.01 \\
Ivy & 0.41 & 0.01 & 0.39 & 0.02 &  &  & 0.43 & 0.03 & 0.33 & 0.01 & 0.38 & 0.02 & 0.37 & 0.01 & 0.51 & 0.04 & 0.35 & 0.01 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.01 \\
Poi & 0.6 & 0.03 & 0.54 & 0.02 & 0.57 & 0.03 &  &  & 0.59 & 0.03 & 0.42 & 0.04 & 0.33 & 0.01 & 0.66 & 0.03 & 0.36 & 0.01 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.01 \\
Velocity & 0.49 & 0.02 & 0.42 & 0.01 & 0.64 & 0.01 & 0.67 & 0.01 &  &  & 0.54 & 0.01 & 0.44 & 0.02 & 0.73 & 0.02 & 0.51 & 0.01 & \cellcolor[HTML]{E8E8E8}0.49 & \cellcolor[HTML]{E8E8E8}0.01 \\
Xalan & 0.56 & 0.01 & 0.52 & 0.02 & 0.62 & 0.02 & 0.59 & 0.01 & 0.56 & 0.01 &  &  & 0.46 & 0.01 & 0.66 & 0.01 & 0.46 & 0.01 & \cellcolor[HTML]{E8E8E8}0.45 & \cellcolor[HTML]{E8E8E8}0 \\
Xerces & 0.71 & 0.01 & 0.51 & 0.01 & 0.67 & 0.01 & 0.62 & 0.02 & 0.62 & 0.01 & 0.55 & 0.01 &  &  & 0.71 & 0.01 & 0.49 & 0.01 & \cellcolor[HTML]{E8E8E8}0.48 & \cellcolor[HTML]{E8E8E8}0.01 \\
Jedit & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.01 & 0.38 & 0.01 & 0.48 & 0.01 & 0.37 & 0.01 & 0.47 & 0.01 & 0.28 & 0 & 0.37 & 0 &  &  & 0.31 & 0.01 & 0.34 & 0.01 \\
Log4j & 0.62 & 0.01 & 0.42 & 0.01 & 0.59 & 0.01 & 0.56 & 0 & 0.39 & 0.01 & 0.53 & 0.02 & \cellcolor[HTML]{E8E8E8}0.39 & \cellcolor[HTML]{E8E8E8}0 & 0.68 & 0.03 &  &  & 0.49 & 0.03 \\ \hline
\end{tabular}%
}\\[0.5cm]
%
%
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ll|ll|ll|ll|ll}
 & \multicolumn{2}{c|}{CM} & \multicolumn{2}{c|}{JM} & \multicolumn{2}{c|}{KC} & \multicolumn{2}{c|}{MW} & \multicolumn{2}{c}{MC} \\ \cline{2-11} 
 & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr & Med & Iqr \\ \hline
CM &      &   & 0.41 & 0 & 0.69 & 0 & 0.49 & 0 & \cellcolor[HTML]{E8E8E8}0.37 & \cellcolor[HTML]{E8E8E8}0 \\
JM & 0.77 & 0 &  &  & 0.65 & 0 & 0.69 & 0 & \cellcolor[HTML]{E8E8E8}0.38 & \cellcolor[HTML]{E8E8E8}0 \\ 
KC & 0.79 & 0 & 0.44 & 0 &  &  & 0.59 & 0 & \cellcolor[HTML]{E8E8E8}0.4 & \cellcolor[HTML]{E8E8E8}0 \\ 
MW & 0.62 & 0 & 0.57 & 0 & 0.41 & 0 &  &  & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0 \\\hline
\end{tabular}%
~~~~\begin{tabular}{l|ll|ll|ll|ll|ll}
    & \multicolumn{2}{c|}{EQ} & \multicolumn{2}{c|}{JDT} & \multicolumn{2}{c|}{ML} &  \multicolumn{2}{c|}{PDE} & \multicolumn{2}{c}{LC} \\ \cline{2-11} 
    & Med        & Iqr        & Med         & Iqr        & Med        & Iqr        & Med         & Iqr        & Med        & Iqr        \\ \hline
EQ  &            &            & 0.62        & 0.01       & 0.35       & 0.01       & 0.4         & 0.01       & \cellcolor[HTML]{E8E8E8}0.34       & \cellcolor[HTML]{E8E8E8}0.01       \\ 
JDT & 0.36       & 0.02       &             &            & 0.28       & 0.03       & 0.28        & 0.01       & \cellcolor[HTML]{E8E8E8}0.28       & \cellcolor[HTML]{E8E8E8}0          \\ 
ML  & 0.42       & 0.01       & 0.51        & 0.02       &            &            & 0.39        & 0.02       & \cellcolor[HTML]{E8E8E8}0.37       & \cellcolor[HTML]{E8E8E8}0.01       \\ 
PDE & \cellcolor[HTML]{E8E8E8}0.32       & \cellcolor[HTML]{E8E8E8}0.01       & 0.54        & 0.01       & 0.34       & 0.01       &             &            & 0.36       & 0.01  \\ \hline    
\end{tabular}%
~~~~\begin{tabular}{l|l|l|l|l|l|l}
       & \multicolumn{2}{c|}{Apache} & \multicolumn{2}{c|}{ZXing} & \multicolumn{2}{c}{Safe} \\ \cline{2-7} 
       & Med           & Iqr         & Med          & Iqr         & Med          & Iqr        \\ \hline
Apache &               &             & 0.51         & 0.09        & \cellcolor[HTML]{E8E8E8}0.46         & \cellcolor[HTML]{E8E8E8}0   \\       

Zxing  & 0.79          & 0           &              &             & \cellcolor[HTML]{E8E8E8}0.51         & \cellcolor[HTML]{E8E8E8}0         \\\hline
\end{tabular}
%
}
\caption{Identifying the ``Bellwether'', This figure compares the prediction performance of the bellwether (highlighted in \textbf{bold}) against other datasets.  ``Med'' refers to the median value seen in 40 repeats.
``IQR'' refers to the 75th-25th percentile seen in those 40 repeats
(and the IQR is very small).
All performance figures here are the ED from \eq{ED} so {\em lower} values
are {\em better}.}
\label{fig:jur1}
\end{figure*}

==> tex/rq11.tex <==
\begin{figure*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{{Ant}} &  & & & \\\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.28  &  0.0 & \quart{65}{0}{65}{235} \\
  1 &          poi &    0.28  &  0.0 & \quart{65}{0}{65}{235} \\
  1 &     velocity &    0.28  &  0.02 & \quart{65}{5}{65}{235} \\
  1 &        log4j &    0.28  &  0.02 & \quart{65}{5}{65}{235} \\
  1 &       xerces &    0.3  &  0.01 & \quart{70}{2}{70}{235} \\
  1 &        xalan &    0.3  &  0.01 & \quart{70}{2}{70}{235} \\
\hline  2 &          ivy &    0.32  &  0.01 & \quart{75}{2}{75}{235} \\
  2 &        camel &    0.33  &  0.01 & \quart{75}{2}{77}{235} \\
  2 &        jedit &    0.34  &  0.0 & \quart{79}{0}{79}{235} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{Camel} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.4  &  0.01 & \quart{44}{1}{44}{111} \\
\hline  2 &        log4j &    0.42  &  0.02 & \quart{45}{2}{46}{111} \\
  2 &       xerces &    0.42  &  0.01 & \quart{46}{1}{46}{111} \\
\hline  3 &     velocity &    0.47  &  0.01 & \quart{51}{1}{52}{111} \\
\hline  4 &        xalan &    0.53  &  0.03 & \quart{56}{3}{58}{111} \\
\hline  5 &          poi &    0.57  &  0.01 & \quart{62}{1}{63}{111} \\
\hline  6 &          ant &    0.61  &  0.0 & \quart{67}{0}{67}{111} \\
  6 &          ivy &    0.62  &  0.02 & \quart{67}{2}{68}{111} \\
\hline  7 &        jedit &    0.71  &  0.01 & \quart{78}{1}{78}{111} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Ivy} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.32  &  0.01 & \quart{48}{1}{48}{150} \\
  1 &     velocity &    0.33  &  0.01 & \quart{48}{1}{49}{150} \\
\hline  2 &        log4j &    0.35  &  0.01 & \quart{51}{1}{52}{150} \\
\hline  3 &       xerces &    0.37  &  0.01 & \quart{54}{1}{55}{150} \\
\hline  4 &        xalan &    0.38  &  0.02 & \quart{54}{3}{57}{150} \\
  4 &        camel &    0.39  &  0.01 & \quart{57}{1}{58}{150} \\
\hline  5 &          ant &    0.41  &  0.02 & \quart{60}{3}{61}{150} \\
\hline  6 &          poi &    0.43  &  0.03 & \quart{63}{4}{64}{150} \\
\hline  7 &        jedit &    0.51  &  0.04 & \quart{73}{6}{76}{150} \\
\hline \end{tabular}}\\[0.1cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Xalan} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.45  &  0.0 & \quart{55}{0}{55}{121} \\
  1 &       xerces &    0.46  &  0.01 & \quart{54}{1}{54}{121} \\
  1 &        log4j &    0.46  &  0.01 & \quart{54}{1}{55}{121} \\
\hline  2 &        camel &    0.52  &  0.02 & \quart{61}{3}{63}{121} \\
\hline  3 &     velocity &    0.56  &  0.01 & \quart{66}{1}{67}{121} \\
  3 &          ant &    0.56  &  0.01 & \quart{67}{2}{67}{121} \\
\hline  4 &          poi &    0.59  &  0.01 & \quart{71}{1}{71}{121} \\
\hline  5 &          ivy &    0.64  &  0.02 & \quart{75}{2}{77}{121} \\
\hline  6 &        jedit &    0.66  &  0.01 & \quart{78}{1}{79}{121} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Xerces} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.48  &  0.01 & \quart{52}{2}{54}{112} \\
\hline  2 &        log4j &    0.49  &  0.02 & \quart{54}{2}{55}{112} \\
\hline  3 &        camel &    0.51  &  0.01 & \quart{57}{1}{57}{112} \\
\hline  4 &        xalan &    0.55  &  0.01 & \quart{60}{1}{61}{112} \\
\hline  5 &     velocity &    0.62  &  0.01 & \quart{68}{1}{69}{112} \\
  5 &          poi &    0.62  &  0.01 & \quart{68}{1}{69}{112} \\
\hline  6 &          ivy &    0.67  &  0.02 & \quart{74}{2}{75}{112} \\
\hline  7 &        jedit &    0.71  &  0.01 & \quart{78}{1}{79}{112} \\
  7 &          ant &    0.71  &  0.0 & \quart{79}{0}{79}{112} \\
\hline 
\end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Poi} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &        \textbf{lucene} &    0.33  &  0.01 & \quart{38}{1}{38}{117} \\
  1 &       xerces &    0.33  &  0.01 & \quart{38}{1}{38}{117} \\
\hline  2 &       log4j &    0.36  &  0.01 & \quart{42}{1}{42}{117} \\
\hline  3 &        xalan &    0.42  &  0.04 & \quart{45}{5}{49}{117} \\
\hline  4 &        camel &    0.54  &  0.02 & \quart{62}{2}{63}{117} \\
\hline  5 &     velocity &    0.59  &  0.03 & \quart{67}{3}{69}{117} \\
  5 &          ivy &    0.57  &  0.03 & \quart{67}{3}{67}{117} \\
  5 &          ant &    0.6  &  0.03 & \quart{67}{3}{70}{117} \\
\hline  6 &        jedit &    0.66  &  0.03 & \quart{76}{3}{77}{117} \\
\hline \end{tabular}}\\[0.1cm]


% \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
% \arrayrulecolor{lightgray}
% \rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
%   1 &        log4j &    0.33  &  0.0 & \quart{41}{0}{41}{124} \\
% \hline  2 &     velocity &    0.35  &  0.01 & \quart{43}{1}{43}{124} \\
%   2 &       xerces &    0.36  &  0.01 & \quart{44}{2}{44}{124} \\
% \hline  3 &        camel &    0.44  &  0.01 & \quart{53}{1}{54}{124} \\
% \hline  4 &        xalan &    0.48  &  0.04 & \quart{57}{5}{59}{124} \\
%   4 &          poi &    0.5  &  0.02 & \quart{61}{2}{62}{124} \\
% \hline  5 &          ivy &    0.55  &  0.01 & \quart{68}{1}{68}{124} \\
%   5 &          ant &    0.56  &  0.0 & \quart{69}{0}{69}{124} \\
% \hline  6 &        jedit &    0.63  &  0.02 & \quart{77}{2}{78}{124} \\
% \hline \end{tabular}}

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Velocity} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &        camel &    0.42  &  0.01 & \quart{45}{1}{45}{108} \\
\hline  2 &       xerces &    0.44  &  0.02 & \quart{46}{2}{47}{108} \\
\hline  3 &          ant &    0.49  &  0.02 & \quart{50}{2}{52}{108} \\
  3 &       lucene &    0.49  &  0.02 & \quart{51}{3}{52}{108} \\
\hline  4 &        log4j &    0.51  &  0.01 & \quart{55}{1}{55}{108} \\
\hline  5 &        xalan &    0.54  &  0.01 & \quart{58}{1}{58}{108} \\
\hline  6 &          ivy &    0.64  &  0.01 & \quart{68}{1}{69}{108} \\
\hline  7 &          poi &    0.67  &  0.02 & \quart{71}{2}{72}{108} \\
\hline  8 &        jedit &    0.73  &  0.02 & \quart{77}{2}{78}{108} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Jedit} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &        xalan &    0.28  &  0.0 & \quart{44}{0}{44}{159} \\
\hline  2 &        log4j &    0.31  &  0.01 & \quart{49}{2}{49}{159} \\
\hline  3 &       lucene &    0.34  &  0.0 & \quart{54}{0}{54}{159} \\
  3 &          ant &    0.35  &  0.02 & \quart{54}{3}{55}{159} \\
\hline  4 &       xerces &    0.37  &  0.0 & \quart{59}{0}{59}{159} \\
  4 &          poi &    0.37  &  0.03 & \quart{55}{5}{59}{159} \\
  4 &        camel &    0.38  &  0.02 & \quart{60}{3}{60}{159} \\
\hline  5 &     velocity &    0.47  &  0.02 & \quart{71}{4}{75}{159} \\
  5 &          ivy &    0.48  &  0.04 & \quart{73}{6}{76}{159} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Log4j} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &     velocity &    0.39  &  0.01 & \quart{44}{1}{45}{117} \\
  1 &       xerces &    0.39  &  0.0 & \quart{45}{0}{45}{117} \\
\hline  2 &        camel &    0.42  &  0.01 & \quart{49}{1}{49}{117} \\
\hline  3 &       lucene &    0.49  &  0.03 & \quart{55}{3}{57}{117} \\
\hline  4 &        xalan &    0.53  &  0.03 & \quart{59}{4}{62}{117} \\
\hline  5 &          poi &    0.56  &  0.0 & \quart{65}{0}{65}{117} \\
\hline  6 &          ivy &    0.59  &  0.03 & \quart{67}{3}{69}{117} \\
\hline  7 &          ant &    0.62  &  0.01 & \quart{72}{2}{72}{117} \\
\hline  8 &        jedit &    0.68  &  0.0 & \quart{79}{0}{79}{117} \\
\hline \end{tabular}}\\[0.5cm]
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{{EQ}} &  & & & \\\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           LC &    0.34  &  0.02 & \quart{41}{3}{43}{126} \\
  1 &           ML &    0.35  &  0.01 & \quart{43}{1}{44}{126} \\
\hline  2 &          PDE &    0.4  &  0.02 & \quart{49}{3}{50}{126} \\
\hline  3 &          JDT &    0.62  &  0.01 & \quart{78}{1}{78}{126} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{JDT} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           LC &    0.28  &  0.0 & \quart{60}{0}{60}{216} \\
  1 &          PDE &    0.28  &  0.01 & \quart{58}{2}{60}{216} \\
  1 &           ML &    0.28  &  0.03 & \quart{60}{7}{60}{216} \\
\hline  2 &           EQ &    0.36  &  0.02 & \quart{75}{4}{77}{216} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{ML} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           LC &    0.37  &  0.01 & \quart{56}{2}{58}{156} \\
\hline  2 &          PDE &    0.39  &  0.02 & \quart{59}{3}{61}{156} \\
\hline  3 &           EQ &    0.42  &  0.01 & \quart{65}{2}{65}{156} \\
\hline  4 &          JDT &    0.51  &  0.01 & \quart{78}{1}{79}{156} \\
\hline \end{tabular}}\\[0.1cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{PDE} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           EQ &    0.32  &  0.0 & \quart{45}{0}{45}{142} \\
\hline  2 &           ML &    0.34  &  0.02 & \quart{47}{2}{48}{142} \\
\hline  3 &           LC &    0.36  &  0.02 & \quart{49}{3}{51}{142} \\
\hline  4 &          JDT &    0.54  &  0.05 & \quart{72}{7}{77}{142} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{LC} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           EQ &    0.27  &  0.01 & \quart{39}{2}{41}{153} \\
\hline  2 &          PDE &    0.34  &  0.02 & \quart{50}{3}{52}{153} \\
\hline  3 &           ML &    0.4  &  0.05 & \quart{56}{8}{61}{153} \\
\hline  4 &          JDT &    0.51  &  0.02 & \quart{76}{3}{78}{153} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{CM} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.37  &  0.0 & \quart{42}{0}{42}{115} \\
  1 &           jm &    0.41  &  0.0 & \quart{47}{0}{47}{115} \\
\hline  2 &           mw &    0.49  &  0.0 & \quart{56}{0}{56}{115} \\
\hline  3 &           kc &    0.69  &  0.0 & \quart{79}{0}{79}{115} \\
\hline \end{tabular}}\\[0.1cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{JM} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.38  &  0.0 & \quart{39}{0}{39}{103} \\
\hline  2 &           kc &    0.65  &  0.0 & \quart{67}{0}{67}{103} \\
\hline  3 &           mw &    0.69  &  0.0 & \quart{71}{0}{71}{103} \\
\hline  4 &           cm &    0.77  &  0.0 & \quart{79}{0}{79}{103} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{KC} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.4  &  0.0 & \quart{40}{0}{40}{101} \\
\hline  2 &           jm &    0.44  &  0.0 & \quart{44}{0}{44}{101} \\
\hline  3 &           mw &    0.59  &  0.0 & \quart{59}{0}{59}{101} \\
\hline  4 &           cm &    0.79  &  0.0 & \quart{79}{0}{79}{101} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{MW} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mc &    0.32  &  0.0 & \quart{41}{0}{41}{129} \\
\hline  2 &           kc &    0.41  &  0.0 & \quart{52}{0}{52}{129} \\
\hline  3 &           jm &    0.57  &  0.0 & \quart{73}{0}{73}{129} \\
\hline  4 &           cm &    0.62  &  0.0 & \quart{79}{0}{79}{129} \\
\hline \end{tabular}}\\[0.5cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Apache} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &         Safe &    0.47  &  0.0 & \quart{72}{0}{72}{153} \\
  1 &        Zxing &    0.51  &  0.09 & \quart{66}{13}{78}{153} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{ZXing} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &         Safe &    0.51  &  0.0 & \quart{51}{0}{51}{101} \\
\hline  2 &       Apache &    0.79  &  0.0 & \quart{79}{0}{79}{101} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Safe} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &        Zxing &    0.3  &  0.03 & \quart{39}{5}{42}{142} \\
\hline  2 &       Apache &    0.56  &  0.0 & \quart{79}{0}{79}{142} \\
\hline \end{tabular}}
\caption{Identifying the ``Bellwether'', This figure compares the prediction performance of the bellwether (highlighted in \textbf{bold}) against other datasets.  ``Med'' refers to the median value seen in 40 repeats.
``IQR'' refers to the 75th-25th percentile seen in those 40 repeats
(and the IQR is very small).
All performance figures here are the ED from \eq{ED} so {\em lower} values
are {\em better}.}
\label{fig:jur1}
\end{figure*}

==> tex/rq12.tex <==
\begin{figure*}[htbp!]
\centering
\begin{minipage}{0.63\linewidth}
\vspace{0.1cm}
\resizebox{\linewidth}{!}{
\textbf{Apache}~~\begin{tabular}{l|c|l|l|l|c|c|l|l|l|c}
\multicolumn{1}{c|}{}  & Ant & Camel & Ivy & Jedit & Log4j & \textbf{Lucene} & Poi & Velocity & Xalan & \multicolumn{1}{c}{Xerces}                 \\ \hline
Ant      &     &       &     &       &       & $\times$     &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Camel    &     &       &     &       &       & $\times$     &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Ivy      &     &       &     &       &       & $\times$     &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Poi      &     &       &     &       &       & $\times$     &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Velocity &     &       &     &       &       & $\times$     &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Xalan    &     &       &     &       &       & $\times$     &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Xerces   &     &       &     &       &       & $\times$     &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Jedit    & $\times$  &       &     &       &       &        &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Lucene   &     &       &     &       & $\times$    &        &     &          &       & \multicolumn{1}{c}{}  \bigstrut\\ \hline
Log4j    &     &       &     &       &       &        &     &          &       & \multicolumn{1}{c}{$\times$} \bigstrut\\
\end{tabular}}
\end{minipage}~~~~~~~~~~~~~~~~\begin{minipage}{0.39\linewidth}
\resizebox{0.09\linewidth}{!}{\textbf{NASA}}~~~~\resizebox{0.5\linewidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\multicolumn{1}{c|}{} & CM & JM & KC & \textbf{MC} & MW \\ \hline
CM &  &  &  & $\times$ &  \bigstrut\\ \hline
JM &  &  &  & $\times$ &  \bigstrut\\ \hline
KC &  &  &  & $\times$ &  \bigstrut\\ \hline
MW &  &  &  & $\times$ &  \bigstrut\\ \hline
MC &  & $\times$ &  &  & 
\end{tabular}}\\[0.1cm]
\resizebox{0.11\linewidth}{!}{\textbf{AEEEM}}~~\resizebox{0.5\linewidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
 & EQ & JDT & \textbf{LC} & ML & PDE \\ \hline
EQ &  &  & $\times$ &  &  \bigstrut\\ \hline
JDT &  &  & $\times$ &  &  \bigstrut\\ \hline
ML &  &  & $\times$ &  &  \bigstrut\\ \hline
PDE & $\times$ &  &  &  &  \bigstrut\\ \hline
LC & $\times$ &  &  &  & 
\end{tabular}}\\[0.1cm]
\resizebox{0.09\linewidth}{!}{\textbf{Relink}}~~~~\resizebox{0.5\linewidth}{!}{
\begin{tabular}{l|l|l|l}
 & Apache & ZXing & \textbf{Safe} \\ \hline
Apache &  &  & $\times$ \bigstrut\\ \hline
ZXing &  &  & $\times$ \bigstrut\\ \hline
Safe &  & $\times$ & 
\end{tabular}}
\end{minipage}
\caption{Identifying the ``Bellwether'' --- This figure summarizes the key findings of \fig{jur1}. As described in \tion{rq1}, we discovered the existence of a bellwether dataset in each of the four groups.}
\label{fig:jur}
\end{figure*}

==> tex/rq2.tex <==
\begin{figure}[!t]
% \arrayrulecolor{lightgray}
\scriptsize
\centering

\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l}
         & Bellw Data \& TCA+                                  & \multicolumn{3}{c}{Local}                                                      \\ \cline{2-5} 
         & \multicolumn{1}{c|}{Lucene}                                            & 
         Train              & Test 
         &                                                     \bigstrut\\
         & \multicolumn{1}{c|}{(G-score)}                                            
         &                    &      & 
         G-Score                                             \bigstrut\\ \hline
         Ant      & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 70}  & 1.6 & 1.7  & 
         64                                                \bigstrut\\
         Camel    & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 63} & 1.4      & 1.6  & 
         57                                                \bigstrut\\
         Xalan    & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 64} & 2.6      & 2.7  & 
         55                                                \bigstrut\\
         Xerces   & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 56} & 1.3      & 1.4  & 
         38                                                \bigstrut\\
         Ivy      & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 72} & 
         1.4           & 2    & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 
         72} \bigstrut\\
         Velocity & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 59} &
         1.5           & 1.6  & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 
         59} \bigstrut\\
         Log4j    & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 61} &
         1.1           & 1.2  & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 
         61} \bigstrut\\
         Jedit    & 57                                                & 4.2 & 4.3  & \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 
         62} \bigstrut\\ \hline
\end{tabular}}
\caption{\respto{2-D} \respto{3-E} Bellwether dataset (Lucene) and TCA+ vs. Local Data.  Performance scores are G-scores so
{\em higher} values are {\em better}.  Note
tthat this best score might be found in both local and bellwether treatments (e.g. see IVY).
Cells highlighted in \colorbox[HTML]{E8E8E8}{gray} indicate datasets with superior prediction capability.
}
\label{fig:rq2}
\end{figure}

==> tex/rq21.tex <==
\begin{figure*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{{Ant}} &  & & & \\\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.3  &  0.01 & \quart{64}{3}{64}{216} \\
\hline  2 &          ant &    0.36  &  0.01 & \quart{77}{2}{77}{216} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray}
\textbf{Camel} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
   1 &       \textbf{lucene} &    0.37  &  0.02 & \quart{65}{4}{67}{181} \\
\hline  2 &        camel &    0.43  &  0.01 & \quart{78}{1}{78}{181} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Ivy} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.28  &  0.01 & \quart{77}{2}{77}{285} \\
  1 &          ivy &    0.28  &  0.03 & \quart{71}{8}{71}{285} \\
\hline \end{tabular}}\\[0.4cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Xalan} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.36  &  0.01 & \quart{60}{2}{62}{173} \\
\hline  2 &        xalan &    0.45  &  0.02 & \quart{76}{3}{78}{173} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Xerces} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.44  &  0.03 & \quart{53}{4}{55}{126} \\
\hline  2 &       xerces &    0.62  &  0.02 & \quart{77}{2}{78}{126} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Poi} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &       \textbf{lucene} &    0.23  &  0.02 & \quart{46}{4}{48}{210} \\
\hline  2 &          poi &    0.36  &  0.06 & \quart{67}{12}{75}{210} \\
\hline \end{tabular}}\\[0.4cm]

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Velocity} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &     velocity &    0.39  &  0.01 & \quart{74}{2}{74}{190} \\
  1 &       lucene &    0.41  &  0.02 & \quart{76}{3}{78}{190} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Jedit} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &        jedit &    0.38  &  0.0 & \quart{70}{0}{70}{186} \\
\hline  2 &       lucene &    0.43  &  0.01 & \quart{78}{1}{79}{186} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{Log4j} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &     velocity &    0.39  &  0.01 & \quart{44}{1}{45}{117} \\
  1 &       xerces &    0.39  &  0.0 & \quart{45}{0}{45}{117} \\
\hline \end{tabular}}\\[0.3cm]
%% NASA
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{CM} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           cm &    0.12  &  0.0 & \quart{22}{0}{22}{190} \\
\hline  2 &           mc &    0.42  &  0.0 & \quart{79}{0}{79}{190} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{JM} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           jm &    0.36  &  0.0 & \quart{75}{0}{75}{210} \\
\hline  2 &           mc &    0.38  &  0.01 & \quart{77}{2}{79}{210} \\
\hline \end{tabular}}\\[.1cm]

\resizebox{0.65\linewidth}{!}{
\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{KC} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           kc &    0.06  &  0.0 & \quart{12}{0}{12}{216} \\
\hline  2 &           mc &    0.37  &  0.01 & \quart{77}{2}{79}{216} \\
\hline \end{tabular}~~~\begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{lightgray} 
\textbf{MW} &  & & & \\[1mm]\hline
\rowcolor{lightgray}\textbf{Rank} & \textbf{Dataset} & \textbf{Median} & \textbf{IQR} & \\\hline
  1 &           mw &    0.05  &  0.0 & \quart{11}{0}{11}{228} \\
\hline  2 &           mc &    0.35  &  0.01 & \quart{77}{2}{79}{228} \\
\hline \end{tabular}}

\caption{}
\label{fig:rq2}
\end{figure*}

==> tex/rq3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\newcommand{\ZZ}{$\cdot$}
\begin{figure*}[htbp!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
         & wmc & dit & noc & cbo & rfc & lcom & ca & ce & npm & lcom3 & loc & dam & moa & mfa & cam & ic & cbm & amc & max\_cc & avg\_cc \\ \hline
ant      & $\times$     & \ZZ     & \ZZ     & $\times$     & \ZZ     & \ZZ      & \ZZ    & \ZZ    & \ZZ     & \ZZ       & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ    & $\times$     & \ZZ     & \ZZ         & \ZZ         \\ \hline
camel    & \ZZ     & $\times$     & \ZZ     & $\times$     & \ZZ     & \ZZ      & \ZZ    & \ZZ    & \ZZ     & \ZZ       & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ    & \ZZ     & \ZZ     & \ZZ         & \ZZ         \\ \hline
ivy      & $\times$     & \ZZ     & \ZZ     & \ZZ     & $\times$     & \ZZ      & $\times$    & \ZZ    & \ZZ     & \ZZ       & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ    & \ZZ     & \ZZ     & \ZZ         & $\times$         \\ \hline
jedit    & $\times$     & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ      & \ZZ    & \ZZ    & \ZZ     & \ZZ       & \ZZ     & $\times$     & \ZZ     & \ZZ     & $\times$     & $\times$    & $\times$     & \ZZ     & \ZZ         & \ZZ         \\ \hline
log4j    & \ZZ     & \ZZ     & \ZZ     & \ZZ     & $\times$     & \ZZ      & \ZZ    & \ZZ    & \ZZ     & \ZZ       & \ZZ     & \ZZ     & \ZZ     & \ZZ     & $\times$     & \ZZ    & \ZZ     & $\times$     & \ZZ         & \ZZ         \\ \hline
poi      & \ZZ     & $\times$     & \ZZ     & \ZZ     & \ZZ     & \ZZ      & $\times$    & $\times$    & \ZZ     & \ZZ       & \ZZ     & $\times$     & \ZZ     & $\times$     & $\times$     & \ZZ    & \ZZ     & \ZZ     & $\times$         & $\times$         \\ \hline
velocity & \ZZ     & $\times$     & \ZZ     & $\times$     & $\times$     & \ZZ      & $\times$    & \ZZ    & $\times$     & \ZZ       & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ    & \ZZ     & \ZZ     & \ZZ         & \ZZ         \\ \hline
xalan    & \ZZ     & \ZZ     & \ZZ     & $\times$     & $\times$     & \ZZ      & \ZZ    & \ZZ    & $\times$     & \ZZ       & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ     & \ZZ    & \ZZ     & \ZZ     & $\times$         & $\times$         \\ \hline
xerces   & $\times$     & $\times$     & \ZZ     & \ZZ     & \ZZ     & \ZZ      & \ZZ    & \ZZ    & \ZZ     & \ZZ       & \ZZ     & \ZZ     & \ZZ     & $\times$     & \ZZ     & \ZZ    & \ZZ     & \ZZ     & \ZZ         & $\times$        
\end{tabular}%
}\\[.3cm]

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%   & Blank & Branch & Code\&Comment & Comments & CC & DC & EC & LOC\_EXE & H_\CONTENT & H\_DIFFICULTY & H\_EFFORT & H\_ERROR & H\_LEN & H\_LVL & H\_PROG & H\_VOL & OPERANDS & OPERATORS & UNIQUE\_OPERANDS & UNIQUE\_OPERATORS & LOC \\ \hline
% cm & \ZZ            & \ZZ               & \ZZ                         & \ZZ               & \ZZ                        & \ZZ                    & \ZZ                       & \ZZ                 & \ZZ                   & \ZZ                      & \ZZ                  & \ZZ                      & \ZZ                  & \ZZ                 & \ZZ                      & \ZZ                  & \ZZ               & \ZZ                & \ZZ                       & \ZZ                        & \ZZ            \\ \hline
% jm & \ZZ            & \ZZ               & \ZZ                         & \ZZ               & \ZZ                        & \ZZ                    & \ZZ                       & \ZZ                 & \ZZ                   & \ZZ                      & \ZZ                  & \ZZ                      & \ZZ                  & \ZZ                 & \ZZ                      & \ZZ                  & \ZZ               & \ZZ                & \ZZ                       & \ZZ                        & \ZZ            \\ \hline
% kc & \ZZ            & \ZZ               & \ZZ                         & \ZZ               & \ZZ                        & \ZZ                    & \ZZ                       & \ZZ                 & \ZZ                   & \ZZ                      & \ZZ                  & \ZZ                      & \ZZ                  & \ZZ                 & \ZZ                      & \ZZ                  & \ZZ               & \ZZ                & \ZZ                       & \ZZ                        & \ZZ            \\ \hline
% mw & \ZZ            & \ZZ               & \ZZ                         & \ZZ               & \ZZ                        & \ZZ                    & \ZZ                       & \ZZ                 & \ZZ                   & \ZZ                      & \ZZ                  & \ZZ                      & \ZZ                  & \ZZ                 & \ZZ                      & \ZZ                  & \ZZ               & \ZZ                & \ZZ                       & \ZZ                        & \ZZ            \\ 
% \end{tabular}%
% }
\caption{Results of Kruskal-Wallis H-Test comparing the 
bellwether dataset (Lucene) with the other datasets from the Apache. Each 
dataset contains 20 Static Code Metrics (for a description of each of these 
metrics, please refer to~\cite{me12d}). The rows contain the test data, and 
the columns contain the metrics. An ``$\times$'' symbol represents a 
significant 
statistical similarity (with a 95\% confidence interval) and a ``$.$'' 
represents a no similarity.}
\label{fig:multcomp}
\end{figure*}

==> tex/rq3_1.tex <==
\begin{figure}[t!]
% \arrayrulecolor{lightgray}
\centering
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{ll|ll|ll|ll}
 &  & \multicolumn{2}{c|}{Bellwether} & \multicolumn{2}{c|}{Turhan09} & \multicolumn{2}{c}{Turhan11} \\ \cline{3-8} 
 &  & Med & Iqr & Med & Iqr & Med & Iqr \\ \hline
\multicolumn{1}{l|}{\multirow{9}{*}{Apache}} & Ant & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.01 & 0.77 & 0.01 & 0.77 & 0.1 \\
\multicolumn{1}{l|}{} & Camel & \cellcolor[HTML]{E8E8E8}0.42 & \cellcolor[HTML]{E8E8E8}0.02 & 0.42 & 0.01 & 0.43 & 0.01 \\
\multicolumn{1}{l|}{} & Ivy & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.01 & 0.4 & 0.01 & 0.41 & 0.01 \\
\multicolumn{1}{l|}{} & Poi & \cellcolor[HTML]{E8E8E8}0.3 & \cellcolor[HTML]{E8E8E8}0 & 0.42 & 0.01 & 0.48 & 0.04 \\
\multicolumn{1}{l|}{} & Velocity & \cellcolor[HTML]{E8E8E8}0.41 & \cellcolor[HTML]{E8E8E8}0.01 & 0.77 & 0 & 0.77 & 0.01 \\
\multicolumn{1}{l|}{} & Xerces & \cellcolor[HTML]{E8E8E8}0.51 & \cellcolor[HTML]{E8E8E8}0.01 & 0.77 & 0.01 & 0.77 & 0 \\
\multicolumn{1}{l|}{} & Jedit & \cellcolor[HTML]{E8E8E8}0.3 & \cellcolor[HTML]{E8E8E8}0.01 & 0.65 & 0.02 & 0.65 & 0.03 \\
\multicolumn{1}{l|}{} & Log4j & 0.48 & 0.01 & \cellcolor[HTML]{E8E8E8}0.43 & \cellcolor[HTML]{E8E8E8}0.01 & 0.57 & 0.06 \\
\multicolumn{1}{l|}{} & Xalan & 0.45 & 0.01 & \cellcolor[HTML]{E8E8E8}0.41 & \cellcolor[HTML]{E8E8E8}0 & 0.42 & 0.01 \\\hline
\multicolumn{1}{l|}{\multirow{4}{*}{AEEEM}} & EQ & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.01 & 0.77 & 0 & 0.77 & 0.01 \\
\multicolumn{1}{l|}{} & JDT & \cellcolor[HTML]{E8E8E8}0.28 & \cellcolor[HTML]{E8E8E8}0.01 & 0.77 & 0.01 & 0.77 & 0.02 \\
\multicolumn{1}{l|}{} & ML & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.02 & 0.77 & 0.01 & 0.77 & 0.03 \\
\multicolumn{1}{l|}{} & PDE & \cellcolor[HTML]{E8E8E8}0.41 & \cellcolor[HTML]{E8E8E8}0 & 0.75 & 0.01 & 0.76 & 0.02 \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Relink}} & Apache & \cellcolor[HTML]{E8E8E8}0.46 & \cellcolor[HTML]{E8E8E8}0.02 & 0.77 & 0 & 0.77 & 0.02 \\
\multicolumn{1}{l|}{} & ZXing & \cellcolor[HTML]{E8E8E8}0.51 & \cellcolor[HTML]{E8E8E8}0.01 & 0.77 & 0.01 & 0.77 & 0.03 \\ \hline
\multicolumn{1}{l|}{\multirow{4}{*}{NASA}} & CM & \cellcolor[HTML]{E8E8E8}0.37 & \cellcolor[HTML]{E8E8E8}0 & 0.69 & 0 & 0.75 & 0.02 \\
\multicolumn{1}{l|}{} & JM & \cellcolor[HTML]{E8E8E8}0.38 & \cellcolor[HTML]{E8E8E8}0 & 0.42 & 0.01 & 0.69 & 0 \\
\multicolumn{1}{l|}{} & KC & \cellcolor[HTML]{E8E8E8}0.4 & \cellcolor[HTML]{E8E8E8}0 & 0.69 & 0 & 0.57 & 0 \\
\multicolumn{1}{l|}{} & MW & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0 & 0.76 & 0.02 & 0.7 & 0 \\\hline
\end{tabular}%
}
\caption{Bellwether vs. Homogeneous Transfer Learning methods (Turhan09~\cite{turhan09} and Turhan11~\cite{turhan11}). All results are ED
so {\em lower} values are {\em better}.
Cells highlighted in \colorbox[HTML]{E8E8E8}{gray} indicate datasets with superior prediction capability.}
\label{fig:rq3_1}
\end{figure}


==> tex/rq3_2.tex <==
\begin{figure}[bt!]
\centering
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\multicolumn{1}{c|}{\multirow{2}{*}{Group}} & \multicolumn{1}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{2}{c|}{\# metrics} & \multicolumn{1}{c}{\multirow{2}{*}{Bellwether}} \bigstrut\\ \cline{3-4}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Significant} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c}{} \\\hline
\multirow{4}{*}{AEEEM} & EQ & 26/61 & 42 & \multirow{4}{*}{LC} \bigstrut\\ \cline{2-4}
 & JDT & 12/61 & 19 &  \bigstrut\\ \cline{2-4}
 & ML & 28/61 & 46 &  \bigstrut\\ \cline{2-4}
 & PDE & 13/61 & 21 &  \bigstrut\\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Relink}} & Apache & 0/26 & 0 & \multirow{2}{*}{Safe} \bigstrut\\ \cline{2-4}
\multicolumn{1}{c|}{} & ZXing & 11/26 & 42 &  \bigstrut\\ \hline
\multirow{9}{*}{Apache} & Ant & 3/20 & 15 & \multirow{9}{*}{Lucene} \bigstrut\\ \cline{2-4}
 & Ivy & 4/20 & 20 &  \bigstrut\\ \cline{2-4}
 & Camel & 2/20 & 10 &  \bigstrut\\ \cline{2-4}
 & Poi & 8/20 & 40 &  \bigstrut\\ \cline{2-4}
 & Jedit & 5/20 & 25 &  \bigstrut\\ \cline{2-4}
 & Log4j & 3/20 & 15 &  \bigstrut\\ \cline{2-4}
 & Velocity & 5/20 & 25 &  \bigstrut\\ \cline{2-4}
 & Xalan & 5/20 & 25 &  \bigstrut\\ \cline{2-4}
 & Xerces & 4/20 & 20 &  \bigstrut\\ \hline
\multirow{4}{*}{NASA} & cm & 0/21 & 0 & \multirow{4}{*}{mc} \bigstrut\\ \cline{2-4}
 & jm & 0/21 & 0 &  \bigstrut\\ \cline{2-4}
 & kc & 0/21 & 0 &  \bigstrut\\ \cline{2-4}
 & mw & 0/21 & 0 & \\ 
\end{tabular}%
}
\caption{Results of Kruskal-Wallis H-Test comparing the bellwether datasets 
with the test datasets. }
\label{fig:kw}
\end{figure}

==> tex/smells_dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\hline
\multirow{2}{*}{Smell Type}    & \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{\# of instances} & \multirow{2}{*}{\# metrics} & \multirow{2}{*}{Nature}  \\ \cline{3-4}
                               &                          & Samples         & Smelly (\%)        &                             &                          \\ \hline
\multirow{11}{*}{Feature Envy} & wct                      & 25              & 18 (72.0)          & \multirow{11}{*}{83}        & \multirow{11}{*}{Method} \\
                               & itext                    & 15              & 7 (47.0)           &                             &                          \\
                               & hsqldb                   & 12              & 8 (67.0)           &                             &                          \\
                               & nekohtml                 & 10              & 3 (30.0)           &                             &                          \\
                               & galleon                  & 10              & 3 (30.0)           &                             &                          \\
                               & sunflow                  & 9               & 1 (11.0)           &                             &                          \\
                               & emma                     & 9               & 3 (33.0)           &                             &                          \\
                               & mvnforum                 & 9               & 6 (67.0)           &                             &                          \\
                               & jasml                    & 8               & 4 (50.0)           &                             &                          \\
                               & xmojo                    & 8               & 2 (25.0)           &                             &                          \\
                               & jhotdraw                 & 8               & 2 (25.0)           &                             &                          \\ \hline
\multirow{11}{*}{God Class}    & fitjava                  & 27              & 2 (7.0)            & \multirow{11}{*}{62}        & \multirow{11}{*}{Class}  \\
                               & wct                      & 24              & 15 (63.0)          &                             &                          \\
                               & xerces                   & 17              & 11 (65.0)          &                             &                          \\
                               & hsqldb                   & 15              & 13 (87.0)          &                             &                          \\
                               & galleon                  & 14              & 6 (43.0)           &                             &                          \\
                               & xalan                    & 12              & 6 (50.0)           &                             &                          \\
                               & itext                    & 12              & 6 (50.0)           &                             &                          \\
                               & drjava                   & 9               & 4 (44.0)           &                             &                          \\
                               & mvnforum                 & 9               & 2 (22.0)           &                             &                          \\
                               & jpf                      & 8               & 2 (25.0)           &                             &                          \\
                               & freecol                  & 8               & 7 (88.0)           &                             &                          \\ \hline
\end{tabular}}
\caption{44 Code smells data sets from 4 smell types.
The \# metrics columns shows the number of metrics that are shared
by all members of that community. }
\label{fig:smells_dataset}
\end{figure}
